SUSTain: Scalable Unsupervised Scoring for Tensors and its Application to Phenotyping

This paper presents a new method, which we call SUSTain, that extends real-valued matrix and tensor factorizations to data where values are integers. Such data are common when the values correspond to event counts or ordinal measures. The conventional approach is to treat integer data as real, and then apply real-valued factorizations. However, doing so fails to preserve important characteristics of the original data, thereby making it hard to interpret the results. Instead, our approach extracts factor values from integer datasets as scores that are constrained to take values from a small integer set. These scores are easy to interpret: a score of zero indicates no feature contribution and higher scores indicate distinct levels of feature importance. At its core, SUSTain relies on: a) a problem partitioning into integer-constrained subproblems, so that they can be optimally solved in an efficient manner; and b) organizing the order of the subproblems' solution, to promote reuse of shared intermediate results. We propose two variants, SUSTain_M and SUSTain_T, to handle both matrix and tensor inputs, respectively. We evaluate SUSTain against several state-of-the-art baselines on both synthetic and real Electronic Health Record (EHR) datasets. Comparing to those baselines, SUSTain shows either significantly better fit or orders of magnitude speedups that achieve a comparable fit (up to 425X faster). We apply SUSTain to EHR datasets to extract patient phenotypes (i.e., clinically meaningful patient clusters). Furthermore, 87% of them were validated as clinically meaningful phenotypes related to heart failure by a cardiologist.

==> content/abstract_phenotyping_oriented.tex <==
\begin{abstract}
Unsupervised phenotyping refers to clustering patients based on groups of medical features defining the patients' clinical state (i.e., phenotypes). Matrix and tensor factorization has been a successful machinery in tackling this problem, especially through the use of Electronic Health Records (EHRs). However, it is still an open challenge to extract the patient phenotypes in a concise, easily-interpretable and clinically-meaningful manner.
\js{The 1st paragraph in the abstract is great, but maybe we can move this into intro in a paragraph called "motivating application". In abstract, we can present from a general method perspective, e.g., matrix and tensor factorization has many data mining successes in unsupervised learning,  however, the coefficients of the factors are often numeric values across large range, which is hard to interpret.}

To tackle this challenge, we developed \mname, a framework extracting the phenotype and patient membership factors as \textit{feature scores}, constrained to take values from a small integer set. \mname admits a straightforward interpretation protocol: a score of zero indicates no feature contribution and higher scores indicate \textit{distinct levels} of feature importance. At the same time, it is easily conceivable by clinicians who are familiar with simple, scoring-based descriptions of clinical status (e.g., risk scores). 
\js{If the abstract makes more method oriented, the previous analogy will be moved to the motivating application in intro as well}

We formulate and experimentally demonstrate how \mname can handle both matrix and tensor inputs, through $\mname_M$ and $\mname_T$ methods respectively. Through an efficient formulation of each integer programming subproblem, our methods are much faster and more scalable than baselines achieving comparable fit. As evaluated on both synthetic and real healthcare datasets, $\mname_M$ achieves comparable fit to an integer matrix factorization baseline, up to \textit{$100\times$ faster} and $\mname_T$ can easily handle large-scale tensor inputs for which the baselines fail. \kimis{to add: experiment on increasing number of patients on CMS} Finally, through a  case study on phenotyping heart failure patients, we demonstrate the interpretability of the extracted scores, which was confirmed by a cardiologist.
\end{abstract}


==> content/intro_phenotyping_oriented.tex <==
\section{Introduction}\label{sec:intro}
Phenotyping refers to the process of identifying sets of measurable disease markers, enabling to perform cohort identification, i.e., separate between cases and control patients for several diseases or disease sub-types of interest~\cite{Yadav2017-of,Richesson2016-ar}. %The traditional way of performing this task involved manual chart reviewing, usually done by nurse abstractors; however, the scale enabled by EHRs renders manual chart review impractical~\cite{Yadav2017-of}. Thus, computational phenotyping algorithms are being employed instead~\cite{Hripcsak2013-lx,Kirby2016-pp}.
%Due to the widespread adoption of Electronic Health Records (EHRs), containing event sequences of multiple patient modalities such as diagnoses, medications and procedures,
The scale enabled by Electronic Health Records (EHRs) renders manual phenotype annotation by experts impractical~\cite{Yu2017ps,Yadav2017-of}. Thus, unsupervised phenotyping algorithms are employed in order to discover the underlying patient phenotypes directly based on their EHR data~\cite{Richesson2016-ar}.

Matrix and tensor factorization have been successfully utilized towards unsupervised EHR-based phenotyping (e.g.,~\cite{Ho2014-ml,Ho2014-mh,Wang2015-pa,Perros2015-te,Joshi2016-kt,Perros2017-dh,Henderson2017-ba}). Consider for example the problem setup of Nonnegative Matrix Factorization (NMF)~\cite{Lee1999-kk} when minimizing the squared Frobenius norm of the error:
\begin{equation}\label{eq:nmf}
\text{min}\left\{ || \M{X} - \M{U} \M{V}^T ||_F^2 \;\middle|\; \M{U} \geq 0, \M{V} \geq 0 \right\}
\end{equation}
In the context of unsupervised phenotyping, $\M{X} \in \mathbb{R}^{M \times N}$ is a non-negative input matrix, whose $\M{X}(i, j)$ cell reflects the activity recorded (e.g., event counts) for the $i$-th (out of $M$) patient with respect to the $j$-th (out of $N$) medical features. Given an input number $R$ of desired phenotypes, the matrix $\M{U} \in \mathbb{R}^{M \times R}$ corresponds to a membership matrix of the patients with respect to the $R$ phenotypes. Finally, the matrix $\M{V} \in \mathbb{R}^{N \times R}$ provides the phenotypes' definition: the non-zero elements of the $r$-th column $\M{V}(:, r)$ reveal the relevant medical features to the $r$-th phenotype. 
% \kimis{tensor mention briefly}

\js{I will argue almost all applications for matrix/tensor factorization, the interpretability is more important than approximation error. I can't actually think of a single app where one just cares for apprx error. So let's rephrase to strengthen our claim. }
In contrast to other application domains of Problem~\ref{eq:nmf} where achieving a low approximation error is the top priority (e.g., recommender systems~\cite{koren2009matrix}), in phenotyping, model interpretability is equally (or even more) crucial. Thus, it is imperative to provide the clinicians with a straightforward protocol of translating the patient membership and phenotype factors. We argue that this task is quite challenging if the factors contain (nonnegative) real values, since the large possible range of values makes it hard to intuitively compare different elements. %assess the relative importance of different factor elements. 
The ad hoc heuristics have been introduced to alleviate the interpretability challenges with limited success: 
\js{shorten the list and remove bullet points as these are not really the main pt from this paper}
\begin{itemize}[leftmargin=*]
\item The data mining practitioner employs a hard thresholding to the ranked list of factor elements, in order to avoid overflowing the clinician with information; this operation though is usually not clinically-grounded.
\item The factor values are hidden altogether by the medical expert and only the ranking of the factor elements is actually preserved (e.g., as happens in~\cite{Ho2014-mh,Wang2015-pa,henderson2017gamaid}).\js{no point of citing, unless we are very sure since these are negative points} Thus, potentially valuable information about the individual elements' level of importance is omitted, due to the lack of a suitable interpretation protocol.
\end{itemize}

\begin{table}[b]
\centering
\small
\begin{tabular}{|c c|}
\hline 
\textit{CKD with Heart Failure phenotype contents} & \textit{Score} \\ \hline  
Chronic Kidney Disease (CKD) & $5$\\ 
Hypertensive heart and/or renal disease & $2$ \\ 
Other specified anemia & $2$ \\  
Diabetes with renal manifestations & $2$ \\ 
Other and unspecified diseases of kidney and ureters & $1$ \\ \hline
\end{tabular}
\caption{\small Chronic Kidney Disease (CKD) with Heart Failure phenotype extracted via $\mname_M$ for a cohort of Heart Failure patients. The score of each diagnostic category indicates its relative prevalence within the phenotype. %In this example, the CKD diagnosis reflects the maximum possible score ($\tau_2 = 5$).
}
\label{table:diab_CKD_ex}
\end{table}

\begin{table}
\centering
\small
\begin{tabular}{|c c|}
\hline 
 \textit{Phenotype name} & \textit{Score} \\ \hline
 CKD with Heart Failure & $5$ \\ 
 Coronary atherosclerosis & $1$ \\
 Hypertension & $1$ \\
 Skin \& opthalmic complications & $1$ \\
 \hline
 \end{tabular}
 \caption{\small Example patient membership vector extracted via $\mname_M$ reflecting the relative persistence of each phenotype throughout the patient's medical history. The phenotype annotations are provided by a medical expert.}
 \label{table:pat_membership}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \hline 
%  0.02  &  0  &  0.01  &  0.0034  &  0.2378  &  0.0042  &       0  &  0.0006   &      0 &   0.0233  &  0.0104 \\  \hline
% \end{tabular}
% \caption{\small pat member}
% \label{table:pat_membership}
\end{table}

%This paper tackles this challenge of improving the interpretability of factorization-based unsupervised phenotyping approaches.
%medical experts are used to deal with simple and concise scoring-based descriptions of clinical status (e.g., risk scores~\footnote{In \href{www.mdcalc.com}{MDCalc}, one can find a vast amount of such scores used in medicine.})~\cite{Ustun2017-ri}. The main intuition behind the development of such scores is simple: the range of the possible values revealing the contribution of each clinical aspect is restricted to a small integer set of consecutive values (e.g., $\{0, 1, \dots, 5\}$). A value of zero indicates no contribution of the feature and higher scores indicate \textit{distinct levels of severity or importance}.

To tackle these challenges, we propose  Scalable Unsupervised Scoring for Tensors (\mname), a framework extracting the phenotype and patient membership factors as \textit{feature scores}, constrained to take values from a small integer set. \mname admits a straightforward interpretation protocol: a score of zero indicates no feature contribution and higher scores indicate \textit{distinct levels} of feature importance. We are motivated to target such an interpretation, since it is easily conceivable by medical experts who are used to deal with simple and concise, scoring-based descriptions of a patient's clinical status (e.g., risk scores~\footnote{In \href{www.mdcalc.com}{MDCalc}, one can find a vast amount of such scores used in medicine.})~\cite{Ustun2017-ri,ustun2017world}. \js{this begs the question why those existing risk scores cannot do what we do here, we need one sentence justification }In order to showcase the conciseness of the extracted factors and the simplicity of our interpretation protocol, in Table~\ref{table:diab_CKD_ex}, we provide a representative phenotype and in Table~\ref{table:pat_membership}, we provide an example patient membership vector extracted via \mname. \js{Table 1 the phenotype name is not generated by our algorithm, so we might want to remove that from the table, Table 2, seems to assume phenotype names are given, so we should elaborate.  }


\mname is general in that it can handle both matrix and tensor inputs, through $\mname_M$ and $\mname_T$ methods respectively, which we formulate in Sections~\ref{sec:meth_sustain_m} and \ref{sec:meth_sustain_t} respectively. Through an efficient formulation of each integer programming subproblem, our methods are both faster and more scalable than baselines achieving comparable fit, as evaluated on both synthetic (publicly-available) and real healthcare datasets. As shown in Figure~\ref{fig:sustain_m_sutter_tradeoff}, $\mname_M$ achieves the same level of accuracy as the most accurate baseline \textbf{up to} $100\times$ \textbf{faster}. Also, $\mname_T$ can handle large-scale tensor inputs for which the baselines fail. \kimis{to add: experiment on increasing number of patients on CMS} Finally, through a  case study on phenotyping heart failure patients, we demonstrate the interpretability of the extracted scores, which was confirmed by a cardiologist.

To promote reproducibility, our code will be open-sourced and for reviewing purposes we provide the following link. \kimis{add link to code}

% \begin{figure}
% 	\centering
% 	\subfigure[{asdasd1}]{\includegraphics[width=1.6in]{results_matrix_figures/Sutter_fit}\label{fig:sutter_m_fit}}
% 	\subfigure[{asdasdasd2}]{\includegraphics[width=1.6in]{results_matrix_figures/Sutter_tradeoff}\label{fig:sutter_m_tradeoff}}
% 	\caption{\small asdasd all}
%     \label{fig:sutter_m_exp}
% \end{figure}
\begin{figure}[t]
\centering
\includegraphics[scale=0.3]{results_matrix_figures/Sutter_tradeoff}
\caption{\small Fit (range $[0, 1]$) vs time trade-off for varying target number of phenotypes $R=\{5, 10, 20, 40\}$, on a patients-by-diagnoses matrix formed of $259$K patients from Sutter Health. $\mname_M$ is as accurate as the most accurate baseline (based on~\cite{W_Chang2008-gt,Breen2012-ld,Dong2017-sy}), but up to $2$ orders of magnitude faster ($R=20$ case: $\approx5.5$ hours vs $\approx3.3$ minutes by $\mname_M$). Also, as compared to a carefully-designed heuristic that performs a scale-and-rounding of the real-valued NMF solution, $\mname_M$ achieves up to $15\%$ higher fit.}
\label{fig:sustain_m_sutter_tradeoff}
\end{figure}


